Mesh Neural Cellular Automata

Texture modeling and synthesis are essential for enhancing the realism of virtual environments. Methods that directly synthesize textures in 3D offer distinct advantages to the UV-mapping-based methods as they can create seamless textures and align more closely with the ways textures form in nature. We propose Mesh Neural Cellular Automata (MeshNCA), a method that directly synthesizes dynamic textures on 3D meshes without requiring any UV maps. MeshNCA is a generalized type of cellular automata that can operate on a set of cells arranged on non-grid structures such as the vertices of a 3D mesh. MeshNCA accommodates multi-modal supervision and can be trained using different targets such as images, text prompts, and motion vector fields. Only trained on an Icosphere mesh, MeshNCA shows remarkable test-time generalization and can synthesize textures on unseen meshes in real time. We conduct qualitative and quantitative comparisons to demonstrate that MeshNCA outperforms other 3D texture synthesis methods in terms of generalization and producing high-quality textures. Moreover, we introduce a way of grafting trained MeshNCA instances, enabling interpolation between textures. MeshNCA allows several user interactions including texture density/orientation controls, grafting/regenerate brushes, and motion speed/direction controls. Finally, we implement the forward pass of our MeshNCA model using the WebGL shading language and showcase our trained models in an online interactive demo, which is accessible on personal computers and smartphones and is available at https://meshnca.github.io.

==> figures/Experiments/comparison-generalization.tex <==
% \newcommand{\motionimg}[1]{\includegraphics[height=60pt]{figures/Experiments/image-motion/#1}}

% \newcommand{\motionimg}[1]{%
%   \ifimgprefix
%     \includegraphics[height=60pt]{figures/Experiments/image-motion/#1}%
%   \else
%     \includegraphics[height=60pt]{figures/Experiments/image-motion/L_#1}%
%   \fi
% }

\begin{table*}[]
\centering
\begin{tabular}{c||c|ccccc}
 \multirow{2}{*}{\textbf{Target}}  &  \multicolumn{6}{c}{\textbf{Methods}}  \\
 
 & Ours & A & B & C &  D & E \\
 \midrule
\imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} \\
\imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} \\
\imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} & \imgimg{test.jpg} \\
\end{tabular}
\captionof{figure}{We are good, they are bad.}
\label{fig:comparison1}
\end{table*}

==> figures/teaser.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\newcommand{\imgteaser}[1]{\includegraphics[height=75pt]{figures/teaser/#1}}
\newcommand{\imgteaserS}[1]{\includegraphics[height=55pt]{figures/teaser/#1}}
\newcommand{\imgteaserM}[1]{\includegraphics[height=68pt]{figures/teaser/#1}}




\begin{table*}[]
\begin{tabular}{m{3pt}F|Gm{0pt}G|||Gm{0pt}G}
    
    
    \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Target Appearance}}} & \multicolumn{3}{c|||}{\hspace{-8pt}\textbf{Target Dynamic}} & \multicolumn{3}{c}{\hspace{-4pt}\textbf{Synthesized result}} \\
    
    \vspace{18pt}
    
    
    &                                    & Video     &        & Optic Flow     & Video      &        & Optic Flow     \\
    \midrule
    
(a) & \imgteaser{bubble_app.jpg}                                & \imgteaserS{none.jpg}      &       & \imgteaserM{target_flow.jpg}            & \imgteaser{bubble_synth.jpg}        & \ofarrow     & \imgteaser{bubble_synth_flow.jpg}            \\


(b) & \imgteaser{flag_app.jpg}                                & \imgteaser{flag_target.jpg}      &     \ofarrow   & \imgteaser{flag_target_flow.jpg}            & \imgteaser{flag_synth.jpg}        & \ofarrow     & \imgteaser{flag_synth_flow.jpg}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (c) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     \ofarrow   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & \ofarrow     & \imgteaser{1.jpeg}            \\

% (d) & \imgteaser{1.jpeg}                                & \imgteaser{1.jpeg}      &     ==   & \imgteaser{1.jpeg}            & \imgteaser{1.jpeg}        & ==     & \imgteaser{1.jpeg}            \\    
\end{tabular}
\caption{1. Difference between optic flow (comparable) 2. Dynamic style transfer on second row}
\end{table*}




==> sections/Experiments/UserStudy.tex <==
% \vspace{-10pt}
\subsection{User Study}
% \vspace{-3pt}
\label{sec:exp-userstudy}
Compare with Text2Mesh of realism. Is this necessary?





==> sections/Experiments/grafting.tex <==
\subsection{Grafting}
% \yx{this is the original version. Rewrite after we have the new method}
An experiment showcasing the similarity between NCA and biological systems is grafting \cite{graft-nca-youtube}. Specifically, two NCAs can cooperate with each other on the same cell state and generate meaningful in-between patterns just like two plants grow together after grafting. However, arbitrary combinations of NCAs often fail on such tasks. The NCAs should originate from a similar starting point so that they tend to be close to each other in the weight space after training, facilitating grafting. To achieve this, we first train a MeshNCA with random initialization. Then, all other MeshNCAs are trained starting from that specific result. By doing so, we ensure most combinations of NCAs generate meaningful grafting results. 

==> sections/methods/OFNet.tex <==
% \subsubsection{Optic Flow Prediction Network}
% \label{sec:ofnet}

The motion loss guides the DyNCA to produce the desired motion. We use the pre-trained \textit{Optic Flow Prediction Network} from \cite{two_stream} to quantify the motion information between two frames. We denote this network as $\mathcal{F}_{OF}$, and the feature map extracted from layer $l$ as $\mathcal{F}^{l}_{OF}$. For different types of target motion sources, namely vector fields and videos, our motion loss takes two different forms, $\mathcal{L}_{mvec}$ and $\mathcal{L}_{mvid}$, respectively. These terms are discussed below.

% For extracting motion information, we use MSOENet introduced in \cite{two_stream}. \yx{how to introduce this thing}

==> tables/comparison_table_thorough.tex <==

\newcommand\RotText[1]{\rotatebox{90}{\parbox{2cm}{\centering#1}}}

% Light Green: #A8E6CF
% Soft Green: #80D4A5
% Mint Green: #56C27A
% Mid Green: #2DB050
% Greenish Yellow: #A3D045
% Yellow: #FFD700
% Orange: #FF8C00
% Dark Red: #8B0000

% Very Light Red: #FFC1C1
% Light Red: #FF8C8C
% Soft Red: #FF5959
% Medium Red: #FF2F2F
% Deep Red: #FF0000
% Darker Red: #B80000
% Dark Red (less intense than previous): #8F0000

% Very Light Green: #B2FFB2
% Light Green: #66FF66
% Medium Green: #33CC33
% Deep Green: #009900
% Darker Green (not overly dark): #006600

\begin{table*}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc|ccccc|cccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Type}} & 
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{\# $\theta$}} &
\multicolumn{5}{c|}{\textbf{General Properties}} &
\multicolumn{6}{c|}{\textbf{Training Properties}} &
\multicolumn{5}{c}{\textbf{Test-time Properties}}  \\
& & & A & B & C & D  & E & F & G & H & I & J & K & L & M & N & O & P \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\parbox{3cm}{\centering \textbf{\hspace{15pt} \small{Solid Textures}}}}}

& Perlin et al. \cite{perlin_noise} & \cellcolor[HTML]{FFFFFF}{$10^1$} & 
\xmark & \cmark & \xmark & \xmark & \xmark & 
N/A & \cmark & \xmark & \xmark & \xmark & \xmark & 
\cmark & \cmark & \cmark & \xmark & \xmark   \\
 
& Kopf et al. \cite{Solid_from_2d} & \cellcolor[HTML]{FFFFFF}{$10^7$} & 
\cmark & \cmark & \xmark & \xmark & \xmark & 
\hmark & \cmark & \xmark & \xmark & \cmark & \xmark & 
\cmark & \xmark & \cmark & \xmark & \xmark \\

& Oechsle et al. \cite{texture-fields} & \cellcolor[HTML]{FFFFFF}{$10^8$} & 
\xmark & \cmark & \cmark & \cmark & \xmark &
\xmark & \hmark & \hmark & \cmark & \cmark & \cmark & 
\cmark & \cmark & \xmark & \xmark & \xmark \\

& Gutierrez et al. \cite{on-demand-solid-texture} & \cellcolor[HTML]{FFFFFF}{$10^7$} & 
\cmark & \cmark & \xmark & \xmark & \xmark & 
\hmark & \cmark & \xmark & \cmark & \cmark & \xmark & 
\cmark & \cmark & \cmark & \xmark & \xmark \\

& Henzler et al. \cite{neural-texture-space, gramgan} & \cellcolor[HTML]{FFFFFF}{$10^7$} & 
\cmark & \cmark & \cmark & \xmark & \xmark & 
\xmark & \cmark & \hmark & \cmark & \cmark & \cmark & 
\cmark & \cmark & \cmark & \xmark & \xmark \\


& Michel et al. \cite{text2mesh} & \cellcolor[HTML]{FFFFFF}{$10^7$} &
\cmark & \xmark & \hmark & \cmark & \xmark & 
\hmark & \xmark & \xmark & \cmark & \cmark & \xmark & 
\cmark & \xmark & \xmark & \xmark & \xmark \\

% Continue filling in the rest of the rows...
\midrule

\multirow{5}{*}{\rotatebox{90}{\parbox{3.5cm}{\centering \textbf{\hspace{36pt} \small{Surface Texture}}}}} 

& Turk et al. \cite{turk2001texture} & \cellcolor[HTML]{FFFFFF}{$10^5$} & 
\cmark & \xmark & \xmark & \xmark & \xmark & 
\xmark & \xmark & \xmark & \xmark & \cmark & \xmark & 
\xmark & \xmark & \xmark & \xmark & \xmark \\
 % & Li-Yi Wei et al. \cite{li_yi_wei_2000} & $10^5$ & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
 % & Ying et al. \cite{ying_2001} & $10^5$ & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\

& Zhang et al. \cite{progressively-variant-textures} & \cellcolor[HTML]{FFFFFF}{$10^5$} &
\cmark & \xmark & \cmark & \xmark & \xmark & 
\hmark & \xmark & \xmark & \xmark & \cmark & \xmark & 
\xmark & \xmark & \xmark & \xmark & \xmark \\

& Han et al. \cite{fast-example-2dto3d-texture} & \cellcolor[HTML]{FFFFFF}{$10^5$} & 
\cmark & \xmark & \xmark & \xmark & \cmark & 
\cmark & \xmark & \xmark & \xmark & \cmark & \xmark & 
\cmark & \xmark & \xmark & \xmark & \cmark \\



& Siddiqui et al. \cite{texturify} & \cellcolor[HTML]{FFFFFF}{$10^8$} & 
\xmark & \xmark & \cmark & \cmark & \xmark & 
\xmark & \hmark & \xmark & \cmark & \xmark & \cmark & 
\cmark & \cmark & \xmark & \xmark & \xmark \\

& Bokhovkin et al. \cite{mesh2tex} & \cellcolor[HTML]{FFFFFF}{$10^8$} & 
\xmark & \xmark & \cmark & \cmark & \xmark & 
\xmark & \hmark & \hmark & \cmark & \xmark & \cmark & 
\cmark & \cmark & \xmark & \xmark & \xmark \\

% % Continue filling in the rest of the rows...
% \midrule

% Text2Tex \cite{text2tex_2023} & None & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \hmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% TEXTure \cite{texture_2023} & None & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \hmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\

% Continue filling in the rest of the rows...
\midrule

\multirow{6}{*}{\rotatebox{90}{\parbox{3cm}{\centering \textbf{\hspace{10pt} \small{Cellular Automata}}}}}

& Turk et al. \cite{turk-rd-texture} & \cellcolor[HTML]{FFFFFF}{$10^1$} & 
\xmark & \xmark & \xmark & \xmark & \hmark & 
N/A & \cmark & \xmark & \xmark & \xmark & \xmark & 
\cmark & \cmark & \cmark & \xmark & \hmark \\

& Witkin et al. \ep{remove} \cite{rd-texture-uvmapping} & \cellcolor[HTML]{FFFFFF}{$10^1$} &
\xmark & \cmark? & \xmark & \xmark & \hmark& 
N/A & \cmark & \xmark & \xmark & \xmark & \xmark & 
\cmark & \cmark & \cmark & \xmark & \hmark \\

& Fleischer et al. \cite{cellular-texture-generation} & \cellcolor[HTML]{FFFFFF}{$10^2$} & 
\xmark & \xmark & \xmark & \xmark & \cmark & 
N/A & \cmark & \xmark & \xmark & \xmark & \xmark & 
\cmark & \cmark & \cmark & \xmark & \cmark \\

& Gobron et al. \cite{3d-surface-ca} & \cellcolor[HTML]{FFFFFF}{$10^1$} & 
\xmark & \cmark & \xmark & \xmark & \hmark & 
N/A & \cmark & \xmark & \xmark & \xmark & \xmark & 
\cmark & \cmark & \xmark & \xmark & \xmark \\

& Mordvintsev et al. \cite{diff-program-rdsystem} & \cellcolor[HTML]{FFFFFF}{$10^4$} &
\cmark & \xmark & \xmark & \xmark & \hmark & 
\hmark & \cmark & \xmark & \cmark & \cmark & \xmark & 
\cmark & \cmark & \xmark & \xmark & \hmark \\

& \textbf{MeshNCA (Ours)} & \cellcolor[HTML]{FFFFFF}{$10^4$} & 
\cmark & \xmark & \cmark & \xmark & \cmark & 
\hmark & \cmark & \xmark & \cmark & \cmark & \xmark & 
\cmark & \cmark & \cmark & \cmark & \cmark \\


\bottomrule
\end{tabular}
}
\caption{Comparison of 3D texture synthesis methods. 
\textbf{(A)} Can synthesize a diverse set of textures 
\textbf{(B)} Does need high poly meshes 
\textbf{(C)} Allows texture interpolation 
\textbf{(D)} Allows semantic (part-aware) texture synthesis
\textbf{(E)} Can produce dynamic textures on 3D meshes 
\textbf{(F)} Is fast to train
\textbf{(G)} Does not need re-training for a new mesh
\textbf{(H)} Does not need re-training for a new texture
\textbf{(I)} Is differentiable and can be trained end-to-end
\textbf{(J)} Can be trained on a single texture instance
\textbf{(K)} Can be trained on a dataset of textures 
\textbf{(L)} Allows real-time synthesis
\textbf{(M)} Can synthesize new texture instances without re-training
\textbf{(N)} Allows re-orienting the texture on the 3D mesh
\textbf{(O)} Allows texture grafting
\textbf{(P)} Allows controlling motion direction and speed.\ep{define the number of parameters}
\label{tab:method-compare}
}
\end{table*}







==> tables/performance_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
% \begin{tabular}[c]{@{}c@{}}\textbf{Sketch Synthesis} \\ \textbf{Algorithms}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}{Method}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}{Training time/frame}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}{Synthesizing time/frame}\end{tabular} 
&\begin{tabular}[c]{@{}c@{}}{C}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{D}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{E}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{F}\end{tabular} \\
\begin{tabular}[c]{@{}c@{}}{\textbf{G}}\end{tabular} & \\

\midrule 

Tesfaldet et al. \cite{two_stream} &\xmark & \cmark \\

Xie et al. \cite{xie2017generativeconvnet} &\xmark & \xmark \\

\midrule
\textbf{Ours} & \cmark & \cmark \\
\bottomrule
\end{tabular}
}
% \vspace{-5pt}
\caption{Comparison of the speed of training a dynamic texture synthesis model and synthesizing videos with it.}
\label{tab:sketch_synth_comparison}
\end{table}

% Comparison of GAN-based image editing algorithms by their characteristics. \fbox{\textbf{A}} Works on any Dataset, \fbox{\textbf{B}} No test-time optimization, \fbox{\textbf{C}} Works on any GAN architecture, \fbox{\textbf{D}} Can perform the edit using a single image, \fbox{\textbf{E}} Allows global semantic editing, \fbox{\textbf{F}} Allows localized semantic editing, \fbox{\textbf{G}} Allows editing any object in the image


